Large deviation results for triangular arrays of semiexponential random variables

Asymptotics deviation probabilities of the sum S n = X 1 + $\times$ $\times$ $\times$ + X n of independent and identically distributed real-valued random variables have been extensively investigated , in particular when X 1 is not exponentially integrable. For instance, A.V. Nagaev formulated exact asymptotics results for P(S n > x n) when X 1 has a semiexponential distribution (see, [16, 17]). In the same setting, the authors of [4] derived deviation results at logarithmic scale with shorter proofs relying on classical tools of large deviation theory and expliciting the rate function at the transition. In this paper, we exhibit the same asymptotic behaviour for triangular arrays of semiexponentially distributed random variables, no more supposed absolutely continuous.

==> commath.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commandes mathématiques
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\RequirePackage{babel}					%Pour les commandes dépendant de la langue du document
\RequirePackage{amsmath}				%Math de l'AMS
\RequirePackage{amssymb}				%Autres symboles mathématiques
\RequirePackage{amsthm}					%Théorèmes correctement organi}és
\RequirePackage{bbm}					%Fonction indicatrice
\RequirePackage{stmaryrd}				%Crochets pour les intervalles entiers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Rémi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Making \big, etc. a relative size rather than absolute (with default parameters, ex is 4.3045 pt)
%
%\renewcommand\big[1]{{\hbox{$\left#1\vbox to 1.97ex{}\right.\n@space$}}}
%\renewcommand\Big[1]{{\hbox{$\left#1\vbox to 2.67ex{}\right.\n@space$}}}
%\renewcommand\bigg[1]{{\hbox{$\left#1\vbox to 3.37ex{}\right.\n@space$}}}
%\renewcommand\Bigg[1]{{\hbox{$\left#1\vbox to 4.07ex{}\right.\n@space$}}}
%
%% Paired delimiters
%
%\DeclarePairedDelimiter\abs\lvert\rvert % Absolute value
%\DeclarePairedDelimiter\brack\lbrack\rbrack % Brackets
%\DeclarePairedDelimiter\ceil\lceil\rceil % Ceiling
%\DeclarePairedDelimiter\floor\lfloor\rfloor % Floor
%\DeclarePairedDelimiter\intervalicc\llbracket\rrbracket % Closed integer interval
%\DeclarePairedDelimiter\intervalico\llbracket\llbracket % Closed-open integer interval
%\DeclarePairedDelimiter\intervalioc\rrbracket\rrbracket % Open-closed integer interval
%\DeclarePairedDelimiter\intervalioo\rrbracket\llbracket % Open interger interval
%\DeclarePairedDelimiter\norm\lVert\rVert % Norm
%\DeclarePairedDelimiter\paren() % Parentheses
%\DeclarePairedDelimiter\set\{\} % Set
%
%\DeclarePairedDelimiterX\inner[2]\langle\rangle{#1,#2} % Inner product
%\DeclarePairedDelimiterX\intervalcc[2]\lbrack\rbrack{#1,#2} % Closed interval
%\DeclarePairedDelimiterX\intervalco[2]\lbrack\rparen{#1,#2} % Closed-open interval
%\DeclarePairedDelimiterX\intervaloc[2]\lparen\rbrack{#1,#2} % Open-closed interval
%\DeclarePairedDelimiterX\intervaloo[2]\lparen\rparen{#1,#2} % Open interval
%\DeclarePairedDelimiterX\setst[2]\{\}{#1\ \delimsize|\ #2} % Set of the #1 such that #2
%
%% Use of some characters from the Fourier-GUTenberg package
%
%\DeclareFontEncoding{FMS}{}{}
%\DeclareFontSubstitution{FMS}{futm}{m}{n}
%\DeclareFontEncoding{FMX}{}{}
%\DeclareFontSubstitution{FMX}{futm}{m}{n}
%\DeclareSymbolFont{fouriersymbols}{FMS}{futm}{m}{n}
%\DeclareSymbolFont{fourierlargesymbols}{FMX}{futm}{m}{n}
%\DeclareMathDelimiter{\llbracket}{\mathopen}{fouriersymbols}{153}{fourierlargesymbols}{133}
%\DeclareMathDelimiter{\rrbracket}{\mathclose}{fouriersymbols}{154}{fourierlargesymbols}{134}
%\DeclareMathDelimiter{\VERT}{\mathord}{fouriersymbols}{152}{fourierlargesymbols}{147}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Mathématiques générales
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Ensembles de nombres
\newcommand{\ensnombre}[1]{\mathbb{#1}}%
\newcommand{\N}{\ensnombre{N}}
\newcommand{\Z}{\ensnombre{Z}}
\newcommand{\Q}{\ensnombre{Q}}
\newcommand{\R}{\ensnombre{R}}
\newcommand{\C}{\ensnombre{C}}

%Divers
\newcommand{\card}[1]{\left\lvert #1 \right\rvert}

\DeclareMathOperator{\id}{id}

\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norme}[1]{\left\lVert #1 \right\rVert}
\newcommand{\prodscal}[2]{\left\langle {#1} \mathrel{}\middle|\mathrel{} {#2} \right\rangle}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\newcommand{\ensfonction}[3]{#1(#2 ; #3)}
\newcommand{\enstq}[2]{\left\{ #1 \mathrel{}\middle|\mathrel{} #2 \right\}}
\newcommand{\ensavec}[2]{\left\{ #1 \mathrel{};\mathrel{} #2 \right\}}
\newcommand{\enspart}{\mathfrak{P}}

\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\eqdef}{\mathrel{=}:}

\newcommand{\seq}[1]{#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Algèbre linéaire
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ensmatrice}[3]{\mathcal{#1}_{#2}(#3)}

\newcommand{\transposee}[1]{{#1}^\top}
%\newcommand{\transposee}[1]{{}^t\! #1}

\DeclareMathOperator{\Vect}{Vect}
\DeclareMathOperator{\rg}{rg}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Com}{Com}
\DeclareMathOperator{\Mat}{Mat}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Probabilités
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\indic}{\mathbbm{1}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Loi}{\mathcal{L}}
\newcommand{\Espe}{\mathbb{E}}
\newcommand{\ET}{\sigma}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\newcommand{\complementaire}[1]{{}^c\! #1}

\newcommand{\Probcond}[2]{\Prob\left( #1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Loicond}[2]{\Loi\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Especond}[2]{\Espe\left[ #1 \mathrel{}\middle|\mathrel{} #2 \right]}
\newcommand{\Varcond}[2]{\Var\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}




\iflanguage{french}%
{
%VERSION FRANCAISE

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\cosh\relax
\DeclareMathOperator{\cosh}{ch}
\let\sinh\relax
\DeclareMathOperator{\sinh}{sh}
\let\tanh\relax
\DeclareMathOperator{\tanh}{th}

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\arcosh}{argch}
\DeclareMathOperator{\arsinh}{argsh}
\DeclareMathOperator{\artanh}{argth}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intervalle}[4]{\left#1#2\mathclose{}\mathpunct{},#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{]}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{[}}%
\newcommand{\intervalleoo}[2]{\intervalle{]}{#1}{#2}{[}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}%
\newtheorem{theorem}{Théorème}%
\newtheorem{lemma}{Lemme}%
%\newtheorem{lemma}[theorem]{Lemme}%
%\newtheorem{lemma}[section]{Lemme}%
\newtheorem{corollary}{Corollaire}%
\newtheorem{proposition}{Proposition}%
\newtheorem{property}{Propriété}%
\newtheorem{properties}{Propriétés}%
%
\theoremstyle{definition}%
\newtheorem{definition}{Définition}%
\newtheorem{hypothesis}{Hypothèse}%
\newtheorem{example}{Exemple}%
\newtheorem{examples}{Exemples}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remarque}%
\newtheorem*{plus}{Complément}%
\theoremstyle{plain}%
}
{
%VERSION ANGLAISE

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\arcosh}{arcosh}
\DeclareMathOperator{\arsinh}{arsinh}
\DeclareMathOperator{\artanh}{artanh}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intervalle}[4]{\left#1#2,#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{(}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{)}}%
\newcommand{\intervalleoo}[2]{\intervalle{(}{#1}{#2}{)}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%\newcounter{intervallent}%
%\newcommand{\intervallentff}[2]{%
%	\setcounter{intervallent}{#1}%
%	\stepcounter{intervallent}%
%	\left\{#1,\theintervallent,\dots,#2\right\}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\theoremstyle{plain}%
\newtheorem{theorem}{Theorem}%
%
%\theoremstyle{definition}%
\newtheorem{lemma}[theorem]{Lemma}%
%\newtheorem{lemma}[theorem]{Lemma}%
%\newtheorem{lemma}[section]{Lemma}%
\newtheorem{corollary}[theorem]{Corollary}%
\newtheorem{proposition}[theorem]{Proposition}%
\newtheorem{definition}[theorem]{Definition}%
\newtheorem{property}[theorem]{Property}%
\newtheorem{properties}[theorem]{Properties}%
\newtheorem{hypothesis}[theorem]{Assumption}%
%\newtheorem{example}[theorem]{Exemple}%
\newtheorem{examples}[theorem]{Exemples}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remark}%
\newtheorem*{plus}{Plus}%
}
